When Automata Meet Streams: Temporal Logic Compilation for Stream-Based Robotics Task and Motion Planning

Stream-based robotics Task and Motion Planning (TAMP) integrates discrete symbolic planning with dynamically generated continuous geometric parameters, such as poses, grasps, and trajectories. However, stream-based planners typically reason only about goal reachability, whereas long-horizon tasks also demand adherence to temporal specifications, such as safety-critical ordering, invariance, and liveness constraints. No methods currently exist to enforce such temporal constraints for stream-based solvers because streams generate an expanding geometric object set via iterative stream refinement loops during planning, rendering existing temporal-logic compilation techniques incompatible. We therefore present Synchronous Action Monitoring with Token Destruction (SAM-TD), a compilation method that enforces arbitrary Linear Temporal Logic over finite traces ($\textrm{LTL}_f$) specifications in stream-based TAMP. SAM-TD translates arbitrary $\textrm{LTL}_f$ constraints into automata and embeds regressed automaton guards into action schemas, which are pre-specified before planning begins. By doing so, SAM-TD can handle objects generated by streams during planning, thus circumventing the need to enumerate a fixed object set or modify the underlying planner. During search, SAM-TD synchronously updates automaton states and uses a validity token shared across all automata to prune constraint-violating branches. We show that SAM-TD supports dynamically generated stream objects from iterative stream refinements during plan search. Experimental results provide the first ever demonstration of stream-based TAMP under $\textrm{LTL}_f$ constraints in three robotics PDDLStream environments. Furthermore, on standard discrete PDDL benchmarks, SAM-TD is competitive with state-of-the-art temporal-constraint compilation methods.

==> titleblock_anon.tex <==
% =====================================================================
% titleblock_anon.tex -- title block for the ANONYMOUS submission.
%
% The [submission] option to aaai2027.sty already suppresses \author and
% \affiliations and prints "Anonymous submission" instead. The real names
% are additionally removed from the source here so that they cannot leak
% into the PDF via string search or metadata.
% =====================================================================

% Your title must be in mixed case, not sentence case.
% That means all verbs (including short verbs like be, is, using, and go),
% nouns, adverbs, adjectives should be capitalized, including both words in
% hyphenated terms, while articles, conjunctions, and prepositions are lower
% case unless they directly follow a colon or long dash.
\title{When Automata Meet Streams: Temporal Logic Compilation for \\ Stream-Based Robotics Task and Motion Planning}

\author{
    Anonymous submission
}
\affiliations{
    Anonymous affiliation
}

